TartanAir: A Dataset to Push the Limits of Visual SLAM

We present a challenging dataset, the TartanAir, for robot navigation tasks and more. The data is collected in photo-realistic simulation environments with the presence of moving objects, changing light and various weather conditions. By collecting data in simulations, we are able to obtain multi-modal sensor data and precise ground truth labels such as the stereo RGB image, depth image, segmentation, optical flow, camera poses, and LiDAR point cloud. We set up large numbers of environments with various styles and scenes, covering challenging viewpoints and diverse motion patterns that are difficult to achieve by using physical data collection platforms. In order to enable data collection at such a large scale, we develop an automatic pipeline, including mapping, trajectory sampling, data processing, and data verification. We evaluate the impact of various factors on visual SLAM algorithms using our data. The results of state-of-the-art algorithms reveal that the visual SLAM problem is far from solved. Methods that show good performance on established datasets such as KITTI do not perform well in more difficult scenarios. Although we use the simulation, our goal is to push the limits of Visual SLAM algorithms in the real world by providing a challenging benchmark for testing new methods, while also using a large diverse training data for learning-based methods. Our dataset is available at \url{http://theairlab.org/tartanair-dataset}.

==> trajectory <==
\subsubsection{Trajectory primitives}
For low-level planning, we design several trajectory primitives off-line. With these trajectories, the robot can efficiently move to adjacent buttons. 

accurately move a distance $d$ to left, right, up, down. $d$ represents button spacings.

It is estimated online based on the pose estimation result. The robot can also choose to move forward $a_f$ for a close inspection or move backward $a_f$ to gain more prior knowledge for planning. 

In practice, the robot will firstly build a local map with range sensors that are mounted on its main body, then it will initialize  position and orientation to  


$A$ is the action set with the eight motion primitives, $\{a_l, a_r, a_u, a_d, a_f, a_b\}$. Suppose those are all feasible primitive trajectories, each of which will move the robot arm a distance $l$ along corresponding directions. The tip frame of the robot arm is dynamically adjusted to keep itself parallel with the elevator panel and $l$ is also dynamically determined according to the pose estimation result.

